A Deep Neural Networks ensemble workflow from hyperparameter search to inference leveraging GPU clusters

Automated Machine Learning with ensembling (or AutoML with ensembling) seeks to automatically build ensembles of Deep Neural Networks (DNNs) to achieve qualitative predictions. Ensemble of DNNs are well known to avoid over-fitting but they are memory and time consuming approaches. Therefore, an ideal AutoML would produce in one single run time different ensembles regarding accuracy and inference speed. While previous works on AutoML focus to search for the best model to maximize its generalization ability, we rather propose a new AutoML to build a larger library of accurate and diverse individual models to then construct ensembles. First, our extensive benchmarks show asynchronous Hyperband is an efficient and robust way to build a large number of diverse models to combine them. Then, a new ensemble selection method based on a multi-objective greedy algorithm is proposed to generate accurate ensembles by controlling their computing cost. Finally, we propose a novel algorithm to optimize the inference of the DNNs ensemble in a GPU cluster based on allocation optimization. The produced AutoML with ensemble method shows robust results on two datasets using efficiently GPU clusters during both the training phase and the inference phase.

==> text_2_problem_statement.tex <==
\section{Problem statement}
\label{section:hetero}

\subsection{Hyperparameter optimization}

% definir HPO 
The empirical nature of research in Deep Learning leads scientists to try many model architecture settings, optimization settings and pre-processing settings to find the best suited one for data. Hyperparameters are here represented as a fixed-length vector $\lambda$ encoding the DNN.


Any model previously trained of hyperparameter $\lambda$ sampled from hyperparameter space $\Lambda$ is written $M_{\lambda}$. The hyperparameter optimization goal defined in equation~\ref{eq:hpo} consists in finding the best hyperparamer $\lambda*\in\Lambda$ building a model to reduce the error measured by $E$. The error is measured on the validation data $x_{valid}$ matching labels $y_{valid}$.
\begin{equation}
    \lambda * = \argmin_{\lambda\in\Lambda} E(M_{\lambda}(x_{valid}),y_{valid}) 
    \label{eq:hpo}
\end{equation}



\subsection{Ensemble selection under constraint}
\label{sec:formatenssele}

% Library to do averaging
The previous optimization process will train and evaluate many models $M_{\lambda\in\Lambda}$ which are added in the list $L$ (or "the library"). Let $a\in\{0,1\}^{|L|}$ a vector of size $|L|$ which control for each model $\lambda$ if it is selected ($a_\lambda=1$) or not ($a_\lambda=0$). The combination by averaging of model’s predictions selected by the vector $a$ is given by the equation \ref{eq:avg}
\begin{equation}
    y_{a}=\frac{1}{\sum{a}}\sum_{\lambda\in\Lambda}{a_\lambda M_\lambda(x)}
    \label{eq:avg}
\end{equation}

% Cost of an ensemble
In this paper we define the cost as the inference time expressed in seconds to predict on 10K images. Other costs may be used, like the memory footprint, the power consumption and so on. The ensemble computing cost is given by the formula \ref{eq:costb} where $c_{\lambda}$ is the cost of the model built with hyperparameter $\lambda$. The sum of the cost of models in the ensemble must honour the budget $B$ for the solution $a$ to be valid.
\begin{equation}
    C_{a} = \sum_{\lambda\in\Lambda}  a_{\lambda} c_{\lambda}  s.t.   C_{a} \leq B
    \label{eq:costb}
\end{equation}


% Penalty
To run usual mono-objective HPO algorithms, the constraint is introduced in the (mono)-objective function via penalty
terms \ref{eq:cost} to intensify the
search on feasible zones where the budget is honoured. When the budget is not, the penalty is made of addition of 2 terms. First $\rho_{1}$ allow to ensure us that the global optimum is located on the feasible space boundary. In practice, $\rho_{1}=10$ value is superior to the values returned by $E$.
The second penalty term is "$\rho_{2}(B-C_{a})^{\rho_{3}}$". It is of common
knowledge that the convergence towards feasible space will be more efficient if the penalization expression is related to the amount of constraint violation. $\rho_{2}=1$ is arbitrary chosen ($\rho_{2}=0$ leads to a long-time search in the unfeasible zone). It is also a common choice for better convergence to express the penalty under a quadratic form $\rho_{3}=2$.
\begin{equation}
    penalty_{a} = 
\begin{cases}
    \rho_{1} + \rho_{2}(B-C_{a})^{\rho_{3}}, & \text{if } C_{a} > B\\
    0,              & \text{otherwise}
\end{cases}
\label{eq:cost}
\end{equation}


% Formalisme
The ensemble selection can be therefore written such a function optimization~\ref{eq:ensmin}. To avoid error, the empty ensemble ($\sum{a}=0$) returns the score $+\infty$ without evaluating the formula.
\begin{equation}
a*=\argmin_{a\in{\{0,1\}}^{|L|}} E(y_{a},y) + penalty_{a}
\label{eq:ensmin}
\end{equation}

% Computational complexity
The problem of finding the best ensemble among a library of models of size $n$ produces $2^{n}$ possibilities. We can imagine that for each model we have one bit to enable or disable it. No known exact method except brut forcing all possibilities exist. Due to this combinatorial explosion, we understand the need of an approximate algorithm.




\subsection{GPUs allocation for inference}
\label{sec:gpuallocfor}



% Problem est plus complique
When an ensemble of DNNs is generated we can deploy it on an inference server. However allocating CPUs and GPUs to those DNNs is not a trivial problem in the case where the number of DNNs is greater than the number of GPUs. First, DNNS are heterogenous and the performance of co-localized DNNs into one GPU is complex. Then, the batch size affect the internal parallelism of DNNs and their memory consumption so it needs to be carefully calibrated to maximize the speed and to fit the memory. All those settings may interact between each other in a complex way, that is why multiple benchmarks to optimize the allocation and the batch size is required for a given ensemble of DNNs and infrastructure.

% Memory constraint
Obviously, any allocation provided must fit the DNNs into the available CPUs and GPUs memory to be ready to answer to an end-user request. Additionally, the image per second is the chosen objective to maximize. Therefore, to efficiently serve an end-user we formulate the problem to optimize the allocation speed under a memory constraint.


The performance of $n$ DNNs with $n$ given batch sizes on some given devices is unknown a priori. Therefore, the allocation strategy must be run by a program benchmarking many combinations on simulated data and returning the optimal allocation. The heterogeneity of devices available, the different DNNs computing requirement and the effect of batch size, make this optimization problem NP-hard.

Let $B$ the number of possible batch values, M the sum of available GPUs and CPUs, and $n$ is the number of models in the ensemble. The number of possible allocations is $(B+M)^{n}$. For example, in some experiments presented in the next sections, an ensemble contains 14 DNNs, we set the possible batch size belonging to $\{8,16,32,64,128,256\}$, we use a node with 6 GPUs and 1 CPU available. It makes $13^{14}\approx3.9*10^{15}$ which shows that all possibilities cannot be assessed. 




